Does external medical review reduce disability insurance inflow?

This paper investigates the effects of introducing external medical review for disability insurance (DI) in a system relying on treating physician testimony for eligibility determination. Using a unique policy change and administrative data from Switzerland, I show that medical review reduces DI incidence by 23%. Incidence reductions are closely tied to difficult-to-diagnose conditions, suggesting inaccurate assessments by treating physicians. Due to a partial benefit system, reductions in full benefit awards are partly offset by increases in partial benefits. More intense screening also increases labor market participation. Existing benefit recipients are downgraded and lose part of their benefit income when scheduled medical reviews occur. Back-of-the-envelope calculations indicate that external medical review is highly cost-effective. Under additional assumptions, the results provide a lower bound of the effect on the false positive award error rate.

==> tables/effect-matrix.bak.tex <==
\begin{table}%[ht]
	\centering
	\caption{Possible effects of medical review on latent types}
	\label{tab:effect-matrix}
		\scriptsize
               \sffamily
             \begin{tabular}{*4{>{\centering\arraybackslash}p{.21\textwidth}}cc}
\addlinespace[1em]
 \textbf{\footnotesize Type}                                         &                                                                                                 & \multicolumn{2}{c}{\textit{\footnotesize Eligible}}                                        &                                                                                                &                                                                                                                  \\      % \cmidrule(lr{.75em}){2-5}
                                                                     &                                                                                                 & \multicolumn{2}{c}{{\tiny $E=1$}}                                                          &                                                                                                &                                                                                                                  \\
                                                                     &                                                                                                 &                                                                                            &                                                                                                &  &                                                                                                               \\
                                                                     &                                                                                                 &                                                                                            &                                                                                                &  &                                                                                                               \\
                                                                     & \textbf{\footnotesize Effect of}                                                                & \textit{\footnotesize perverse}                                                            & \textit{\footnotesize non-perverse}                                                            &  &                                                                                                               \\      % \cmidrule(lr{.75em}){3-4} \addlinespace[2em]
                                                                     & \textbf{\footnotesize medical review}                                                           & {\tiny $h^{1}(t|E=1) < h^{0}(t|E=1)$}                                                     & {\tiny $h^{1}(t|E=1)\geq h^{0}(t|E=1)$}                                                        &  &                                                                                                               \\
                                                                     &                                                                                                 &                                                                                            &                                                                                                &  &                                                                                                               \\
                                                                     &                                                                                                 &                                                                                            &                                                                                                &  &                                                                                                               \\
                                                                     &                                                                                                 & \cellcolor{gray!35}                                                                        & \cellcolor{gray!25}                                                                            &  & \cellcolor{gray!25}                                                                                           \\
 \multirowcell{18}{\textit{\footnotesize Ineligible}\\{\tiny $E=0$}} & \multirowcell{9}{\textit{\footnotesize perverse}\\ {\tiny $h^{1}(t|E=0) > h^{0}(t|E=0)$}}      & \cellcolor{gray!35}E=1 rejected more{~}{~}                                                 & \cellcolor{gray!25}E=1 accepted more                                                           &  & \cellcolor{gray!25}   \\
                                                                     &                                                                                                 & \cellcolor{gray!35}E=0 accepted more                                                       & \cellcolor{gray!25}E=0 accepted more                                                           &  & \cellcolor{gray!25}                                                                                           \\
                                                                     &                                                                                                 & \cellcolor{gray!35}                                                                        & \cellcolor{gray!25}                                                                            &  & \cellcolor{gray!25}                                                                                           \\
                                                                     &                                                                                                 & \cellcolor{gray!35}Increase in false rejections must exceed increase in false acceptances. & \cellcolor{gray!25}Indiscriminate acceptances.                                                 &  & \cellcolor{gray!25}                                                                                           \\
                                                                     &                                                                                                 & \cellcolor{gray!35}                                                                        & \cellcolor{gray!25}                                                                            &  & \cellcolor{gray!25}                                                                                           \\
                                                                     &                                                                                                 & \cellcolor{gray!35}Implausible.                                                            & \cellcolor{gray!25}Incompatible with lower inflow.                                             &  & \cellcolor{gray!25}                                                                                           \\
                                                                     &                                                                                                 & \cellcolor{gray!35}                                                                        & \cellcolor{gray!25}                                                                            &  & \cellcolor{gray!25}\parbox[t]{2mm}{\multirow{-11}{*}{\rotatebox[origin=c]{270}{Irreconcilable with effect.}}} \\
                                                                     &                                                                                                 & \cellcolor{gray!15}                                                                        &                                                                                                &  &                                                                                                               \\
                                                                     & \multirowcell{9}{\textit{\footnotesize non-perverse}\\ {\tiny $h^{1}(t|E=0)\leq h^{0}(t|E=0)$}}  & \cellcolor{gray!15}E=1 rejected more{~}{~}                                                 & E=1 accepted more                                                                              &  & \\
                                                                     &                                                                                                 & \cellcolor{gray!15}E=0 rejected more{~}{~}                                                 & E=0 rejected more{~}{~}                                                                        &  &                                                                                                               \\
                                                                     &                                                                                                 & \cellcolor{gray!15}                                                                        &                                                                                                &  &                                                                                                               \\
                                                                     &                                                                                                 & \cellcolor{gray!15}Indiscriminate rejections, reduced inflow is a mix of both types.       & Reduced inflow by ineligible types may be partially offset by higher inflow of eligible types. &  &                                                                                                               \\
                                                                     &                                                                                                 & \cellcolor{gray!15}                                                                        &                                                                                                &  &                                                                                                               \\
                                                                     &                                                                                                 & \cellcolor{gray!15}Upper bound of effect on award errors identified.                       & Lower bound of effect on award errors identified.                                              &  &                                                                                                               \\
                                                                     &                                                                                                 & \cellcolor{gray!15}                                                                        &                                                                                                &  &                                                                                                               \\
                                                                     &                                                                                                 &                                                                                            &                                                                                                &  &                                                                                                               \\
                                                                     &                                                                                                 & \cellcolor{gray!15}Potentially ruled out by assuming \textit{MTR} for $E=1$.               &                                                                                                &  &                                                                                                               \\
		\end{tabular}
\end{table}

